Report of the Topical Group on Higgs Physics for Snowmass 2021: The Case for Precision Higgs Physics

A future Higgs Factory will provide improved precision on measurements of Higgs couplings beyond those obtained by the LHC, and will enable a broad range of investigations across the fields of fundamental physics, including the mechanism of electroweak symmetry breaking, the origin of the masses and mixing of fundamental particles, the predominance of matter over antimatter, and the nature of dark matter. Future colliders will measure Higgs couplings to a few per cent, giving a window to beyond the Standard Model (BSM) physics in the 1-10 TeV range. In addition, they will make precise measurements of the Higgs width, and characterize the Higgs self-coupling. This report details the work of the EF01 and EF02 working groups for the Snowmass 2021 study.

==> Tex/bsm_now.tex <==
{\color{red} Describe the current limits on a few representative models (probably singlet and 2HDM) and point out that they really only probe new physics scales up to $\sim $2 TeV.}

==> Tex/eft.tex <==
{\color{red} Comment that EFT stuff is in EF04.  Comment on generic scales probed by double Higgs in BSM models.}

==> Tex/simp.tex <==
In a general sense, we would like to have an idea of the high scale for where new physics might be.  One general criteria is 
unitarity\cite{Abu-Ajamieh:2022dtm}.
